Guided Imitation of Task and Motion Planning

While modern policy optimization methods can do complex manipulation from sensory data, they struggle on problems with extended time horizons and multiple sub-goals. On the other hand, task and motion planning (TAMP) methods scale to long horizons but they are computationally expensive and need to precisely track world state. We propose a method that draws on the strength of both methods: we train a policy to imitate a TAMP solver's output. This produces a feed-forward policy that can accomplish multi-step tasks from sensory data. First, we build an asynchronous distributed TAMP solver that can produce supervision data fast enough for imitation learning. Then, we propose a hierarchical policy architecture that lets us use partially trained control policies to speed up the TAMP solver. In robotic manipulation tasks with 7-DoF joint control, the partially trained policies reduce the time needed for planning by a factor of up to 2.6. Among these tasks, we can learn a policy that solves the RoboSuite 4-object pick-place task 88% of the time from object pose observations and a policy that solves the RoboDesk 9-goal benchmark 79% of the time from RGB images (averaged across the 9 disparate tasks).

==> algorithms/plannode.tex <==

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-5mm}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{Planning}
\label{plannode}
\begin{algorithmic}[1]
\REQUIRE Shared queue $Q_{prob}$
\REQUIRE Shared dataset $D_{train}$
\REQUIRE Expert Demonstrator $PLAN()$
\WHILE{not terminated}
\STATE $x_0 \leftarrow$ pop($Q_{prob}$)
\STATE $\tau \leftarrow$ $PLAN(x_0)$
\STATE append($D_{train}, \tau$)
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\vspace{-5mm}

\begin{algorithm}[H]
\caption{Policy Training}
\label{policyopt2}
\begin{algorithmic}[1]
\REQUIRE Shared dataset $D_{train}$
\REQUIRE Shared queue $Q_{roll}$
\REQUIRE Imitation learning procedure $TRAIN()$
\STATE Initialize policy $\pi_{\phi}$
\WHILE{not terminated}
\STATE $\{\tau_i\}_0^N \sim D_{train}$
\STATE $TRAIN(\{\tau_i\}_0^N, \phi)$
\STATE \#\# Collects rollouts
\STATE $\{\hat{\tau}_i\}_0^M$ $\leftarrow$ $\pi_{\phi}$
\STATE push($Q_{roll}, \{\hat{\tau}_i\}_0^M$)
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\end{minipage}%
\end{wrapfigure}

==> algorithms/policyopt.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-25pt}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{Policy Optimization Node}
\label{policyopt}
\begin{algorithmic}[1]
\REQUIRE Shared dataset $D$
\REQUIRE Shared memory $\phi$ // Policy parameters
\REQUIRE Imitation procedure $TRAIN()$
\WHILE{not terminated}
\STATE $\tau = (o^{}_0, u^{}_0, r^{}_0), \dots, (o^{}_T, u^{}_T, r^{}_T)$ $\leftarrow$ $D$
\STATE $\hat{\phi}$ $\leftarrow$ $TRAIN(\tau, \phi)$
\STATE Publish $\hat{\phi}$ to $\phi$
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-5pt}

\end{wrapfigure}


==> algorithms/prob.tex <==

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-5mm}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{Problem Sampling}
\label{prob}
\begin{algorithmic}[1]
\REQUIRE Shared queues $Q_{label}$, $Q_{prob}$, $Q_{roll}$
\REQUIRE Shared data $D_{class}$
\REQUIRE Initial problem distribution $P$
\REQUIRE Classifier $C_\theta$ with shared memory $\theta$
\WHILE{not terminated}
\IF{$Q_{label}$ not empty}
\STATE $\{x_0\}, t, $ label $\leftarrow$ pop($Q_{label}$)
\STATE append($D_{class}$, ($x, t, $ label))
\ELSE
\STATE \#\# Samples $P$ if $C_\theta$ is untrained
\STATE $\{x_i\}_0^N \sim C_\phi(P, Q_{roll})$
\ENDIF
\FOR{$x \in \{x_i\}$}
\STATE push($Q_{prob}$, $x$)
\ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\vspace{-5mm}

\begin{algorithm}[H]
\caption{Planning}
\label{plannode}
\begin{algorithmic}[1]
\REQUIRE Shared queue $Q_{prob}$
\REQUIRE Shared dataset $D_{train}$
\REQUIRE Expert Demonstrator $PLAN$
\WHILE{not terminated}
\STATE $x_0 \leftarrow$ pop($Q_{prob}$)
\STATE $\tau \leftarrow$ $PLAN(x_0)$
\STATE append($D_{train}, \tau$)
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\vspace{-5mm}

\begin{algorithm}[H]
\caption{Policy Training}
\label{policyopt2}
\begin{algorithmic}[1]
\REQUIRE Shared dataset $D_{train}$
\REQUIRE Shared queue $Q_{roll}$
\REQUIRE Imitation learning procedure $TRAIN()$
\STATE Initialize policy $\pi_{\phi}$
\WHILE{not terminated}
\STATE $\{\tau_i\}_0^N \sim D_{train}$
\STATE $TRAIN(\{\tau_i\}_0^N, \phi)$
\STATE \#\# Collects rollouts
\STATE $\{\hat{\tau}_i\}_0^M$ $\leftarrow$ $\pi_{\phi}$
\STATE push($Q_{roll}, \{\hat{\tau}_i\}_0^M$)
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\vspace{-5mm}

\begin{algorithm}[H]
\caption{Human Labelling}
\label{labelling}
\begin{algorithmic}[1]
\REQUIRE Shared queues $Q_{label}$, $Q_{roll}$
\WHILE{not terminated}
\STATE $\tau \leftarrow$ pop($Q_{roll}$)
\STATE $\{(x_i, t_i, \text{label}_i)\}_0^N \leftarrow$ LABEL($\tau$)
\STATE push($Q_{label}, \{(x_i, t_i, \text{label}_i)\}_0^N$)
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\vspace{-15mm}
\end{minipage}
\end{wrapfigure}


==> algorithms/tasknode.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-20pt}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\caption{Task Planning Node}
\label{algtask}
\begin{algorithmic}[1]
\REQUIRE Shared queues $Q_{task}, Q_{motion}$
\REQUIRE Problem distribution $P$
\WHILE{not terminated}
\IF {is\_empty($Q_{task}$)}
\STATE $(x_0, \Phi, $g$, \tau) \sim P_{prob}$
\ELSE
\STATE $(x_0, \Phi, $g$, \tau)\ \leftarrow \  $pop$(Q_{task})$
\ENDIF
\STATE $\vec{a} \ \leftarrow \  $task\_plan$(\Phi, g)$
\STATE push($Q_{motion}$, ($x_0$, $\Phi$, g, $\vec{a}$))
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\end{minipage}
%\vspace{-10pt}
\end{wrapfigure}


==> old_eval.tex <==






%============== OLD SECTION BELOW =========================













\subsection{Setup}

%% Add intro paragraph



The final environment is within the RoboDesk benchmark \cite{robodesk}. The controls are the joint velocities of the robot plus the gripper value (for 8 DOF). In this environment, three objects (a ball, an upright block, and a flat block) are randomly initialized on the desk. There are two doors: a drawer at the front of the desk and a slider on the back shelf. For our results, we evaluate on a set of two-goals tasks where the goal set contains an instance for placing each object in the drawer or shelf and an instance for whether or not each door needs ot be closed. The task domain contains six actions: moveto, grasp, place, stack, open\_door, and close\_door.

For our experiments, we used Fast-Forward~\cite{ff} as our symbolic planner and a variant of the trajectory optimizer used by \citet{sqpsolver}. Unless otherwise stated, evaluations of our method used 2 processes for task planning, 18 processes for motion planning, and, when applicable, 10 processes for supervised exploration. 

%Unless otherwise stated, all experiments were run for five random seeds and plots show 500-sample rolling averages with standard deviation. For resource allocation, evaluations of our method used 2 processes for task planning, unless otherwise stated, 18 processes for motion planning, and, when applicable, 10 processes for supervised exploration. Observations in all domains, unless otherwise stated, contained a one-hot encoding of the goal, displacement vectors from the robot gripper to the center of each object, and displacement vectors from the center of each object to its respective goal location. Furthermore, each neural network was trained inside its own process. Further details are in the appendix.

%The first domain has a relatively simple control space but a complex task space, with $\frac{T!}{(T-O)!}$ possible goal configurations. Here $T$ denotes the number of potential target locations and $O$ the number of objects; in the five-object variant this yields 6720 unique possible goals. In contrast, the second domain has a simple task space, as the goals are fixed, but a complicated control space.

\subsection{Acceleration of Task and Motion Planning}


\begin{wrapfigure}{r}{0.45\textwidth}
\begin{minipage}{0.45\textwidth}
\vspace{-50pt}
    \centering
    \includegraphics[width=1.\columnwidth]{figs/tamp_acc.png}
    \caption{Ratio of avg. time for trajectory optimization at the start of training to the avg. time for trajectory optimization at the current time.}
    \label{fig:accexp2}
    \end{minipage}
\vspace{-30pt}
\end{wrapfigure} The primary advantage of learned policies is the ability to instantaneously execute within an environment. Using the robosuite domain as an example, our base planner requires over six minutes on average before it can generate the first action to take. Each neural network requires negligible compute for forward inference, hence no such delay exists when acquiring the first action from the policy. Figure  \ref{fig:accexp2} shows the learned controllers can speedup trajectory optimization (including simulated execution) in our system by a factor of almost 2.


%\cline{2-5} \multicolumn{1}{c|}{}
\begin{wraptable}{r}{0.6\textwidth}
\vspace{-15pt}
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
   &  \multicolumn{2}{c|}{1 object } &  \multicolumn{2}{c|}{2 object }  \\
 \hline
  Method & success rate & distance &  success rate & distance  \\
 \hline
 PPO & 1.3\%& 5.63 &  0\% & 8.46 \\

 Flat & 21\% & 4.05 & 1.5\% & 4.43 \\

 Hierarchy & 99.7\% & 0.11 & 98.7\%& 0.12 \\
 \hline
\end{tabular}
\caption{Comparison of average success rate and distance-to-goal at completion of training for different policy training methods on 2D pickplace problems. Distances are the average l2 distance from each object's final position to its target location. }
\label{fig:rlcomp}
\vspace{-10pt}
\end{wraptable}

\subsection{Comparisons to Reinforcement Learning}
To demonstrate the difficulty of the problem domains we consider, we compare our approach with reinforcement learning. We trained a custom policy in our 2D domain and refer to existing 

first compared our approach with proximal policy optimization (PPO)~\cite{stable-baselines}. We trained in the 2D Pick-Place domain, with a dense reward function that the sums the distance from the robot to the closest object (to incentives grasping) and from each object to its goal. We ran with most of the default hyperparameters and parallelized training over 60 vCPUs. We tuned the number of steps to run each environment per update to be 512 and let training for 9 hours.

As seen in table \ref{fig:rlcomp}, PPO rarely achieved the goal even in the 1 object variant, and never in the 2 object variant. It was only able to move objects modestly towards their goals. The challenges to flat RL here include: (1) proper placement involves deceleration and direction reversal that create sharp discontinuities in the control space, (2) the objects require precise placement relative to the size of the work-space (and are easily knocked off-target by small motions), and (3) the presence of multiple sub-goals inhibits reward shaping. For the robosuite domain (with a single object), we refer to existing benchmarks that show state-of-the-art RL has yet solve this domain.~\citet{surreal} were unable to scale PPO and deep deterministic policy gradients (DDPG) beyond moving a single object. For the one object variant, the official benchmarks for Soft-Actor Critic (SAC) achieve a normalized return below $50$ for 500 timesteps whereas our average returns for the same time horizon ranged from $320$ (with flat policies and no feedback) to over $390$ (with hierarchical policies and combined motion and task feedback)~\cite{robosuite2020}. 

To show the difficulty of learning from offline demonstrations on the robosuite task, we again refer to existing results. In a single object variant of this task, \citet{iris} were able to achieve success rates on the order of $45\%$ using offline human demonstrations from state data, whereas several variants of our approach achieved success rates over $95\%$ as indicated in table \ref{fig:feedcomp}.



\subsection{The Benefit of Hierarchy}


We compare the performance of training with our proposed hierarchy against training a flat policy that maps directly from an observation and goal to controls. Observation and control spaces, along with any hyperparameters unrelated to policy structure, were kept fixed for all evaluations on a task. For these evaluations, all policies had access to state information.

For the robosuite domain with a single object, as seen in table \ref{fig:hiercomp}, hierarchy provided no noticeable benefit in the absence of feedback but provided limited benefit with the presence of feedback. By contrast, the two object variant improved considerably using the hierarchical policy as compared to the flat. In the 2D pick-place domain, hierarchy proved critical. Table \ref{fig:hiercomp} shows the fully-trained flat policy significantly under-performed its hierarchical counterpart when given a single object. With two objects, the flat policy almost never achieved the goal. 

\begin{wraptable}{r}{0.68\textwidth}
\vspace{-10pt}
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Policy &  2D 1-Obj &  2D 2-Obj & RSuite 1-Obj & RSuite 2-Obj \\
 \hline
Flat & 21\% & 1.5\% & 88\% & 14\% \\

Hierarchy & 99.7\% & 98.7\% & 97\% & 90\% \\
 \hline
\end{tabular}

\caption{Comparison average success rate at the end of training for flat and hierarchical policy structures for both 2D navigational and robosuite (RSuite) domains.}
\label{fig:hiercomp}
\vspace{-10pt}
\end{wraptable} 

To shed additional light on these numbers, table \ref{fig:rlcomp}  shows that the hierarchical policy was able to place the objects precisely on the goal. This represents distances approximately 10x closer than the flat policy. While this domain seems simpler than the robosuite domain, it contains several pitfalls uniquely challenging to the flat policy: (1) action transitions involve deceleration and direction reversals that create sharp discontinuities in the control space, which the flat policy does not capture, (2) there are far more possible goals, which increases dependence on the one-hot goal vector when choosing controls, and (3) the objects require precise placement relative to the size of the work-space.



\subsection{The Benefit of Feedback}



\begin{wraptable}{r}{0.60\textwidth}
\vspace{-30pt}
\small
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Variant &  2D 5-obj & RSuite 1-obj & RSuite 2-obj \\
 \hline
No Feedback & 80\% & 58\% & 14\%\\

Task Feedback & n/a & 96\% & 71\%  \\

Motion Feedback & n/a & 97\% & 89\% \\

Full Feedback & 88\% & 97\% & 90\% \\
 \hline
\end{tabular}
\caption{Comparison of average success rate at the end of training with different forms of planner-policy feedback in the system.}
\label{fig:feedcomp}
\vspace{-10pt}
\end{wraptable} We evaluate two forms of feedback in our system: initializing the motion planner at $\pi_{lo}$ and using structured rollouts to generate task problems. For these evaluations, all policies had access to state information. In the 2D pick-place domain, we directly compare full feedback vs. no feedback. As seen in table \ref{fig:feedcomp}, feedback offered only modest benefit to training for the placement of five objects.  For the robosuite domain, we compare four variants: without feedback (essentially behavioral cloning), with only feedback between the motion planner and policy, with only feedback between the task node and the exploration node, and with full task and motion feedback. Motion feedback had a sizable impact within the robosuite domain. As shown in table \ref{fig:feedcomp}, the feedback into the motion planner provided significant performance gains with both one and two objects present. The results in table \ref{fig:feedcomp} show that task-planner feedback (via the exploration node) offered benefit in isolation, but not in the presence of motion-planner feedback. To validate the choice of problem selection, we also ran a variant where random states from the policy rollouts were fed back to the problem distribution. This variant reached a success rate of $48\%$ on the robosuite problem with one object, signficantly lower than the variant with our task feedback. Taken together, these results suggest the benefit of feedback depends more on the dimension of the control space than that of the task space.

%Notably, the TAMP acceleration alone does not explain this gap in performance. As shown in figure \ref{succtime}, the variants with motion planner-policy feedback outperformed those without as a function of the data generated for supervision.


\subsection{Full Evaluation}
We finish by discussing the ability of our system to extend to long horizon tasks in high-dimension observation, task, and control spaces. These results are summarized in figure \ref{fig:topline}. For the robosuite pick-place task, our trained policies can successfully place all four objects 88$\%$ of the time when trained from state data. 



==> old_intro.tex <==

% To reduce distribution shift and accelerate data generation, the trajectory optimizer is initialized around rollouts of the controllers and penalized for deviating from those rollouts in control space. To further facilitate efficient generation of supervision, the components of planning and learning distribute across separate nodes that operate in parallel. Once trained, the policies execute end-to-end and predict both the action encoding and controls at every timestep. This approach uses established machine learning (in particular only feed-forward neural networks) and builds on standard robotics tools.

% Various works have proposed methods to improve TAMP via deep learning. \citet{scorespace} used a score-space representation to guide the search via transferring knowledge from previous plans. \citet{feasibletamp} learned a classifier to assess motion feasibility and incorporated it as a heuristic into the search.  To improve efficiency in trajectory optimization, \citet{gripsqp} trained neural networks to predict approximate trajectories that transition from a start frame to the goal, and used these approximate solutions to warm-start trajectory optimization. All of these approaches do not attempt to acquire executable policies, and hence still require the full planner at execution time.

% In contrast, several works have proposed methods to acquire executable policies that emulate components of TAMP without direct access to an existing planner. In \cite{mctstamp}, the policies trained from scratch through imitation learning of Monte-Carlo Tree Search (MCTS) in an abstract space and deep q-learning in a control space, focusing on low-dimensional controls and un-parameterized actions. To handle more complex problems, \cite{dpdl} proposed a method for imitating hand-crafted solutions to train a high-level model for symbolic state inference alongside low-level controllers to convert symbolic states to controls. Since the model did not predict abstract actions, this structure still requires a symbolic planner be invoked at the start of execution. The approach most similar to ours is \cite{geomlearn}. Using pre-computed TAMP solutions, the authors trained a high-level model to predict both discrete action sequences and associated continuous values in conjunction with a set of controllers. The need to predict full action sequences requires complex, recurrent policy structures with specialized training losses and inhibits extensions to larger task spaces where possible action sequences may grow factorially.



In the past 5 years, (deep) \emph{policy learning} has demonstrated an impressive ability to accomplish robotic control tasks from complex sensory input~\cite{Finn16, trpo, rubiks}. But that success has largely been limited to short-horizon tasks; learning policies that reason over extended sequences of actions remains a challenge~\cite{oneshothier, subpol}. By contrast, \emph{task and motion planning} (TAMP) can solve problems that require hundreds of abstract actions, each consisting of complex geometric constraints in high-dimension configuration spaces~\cite{hiertamp, extendtamp}. Limiting factors on these methods instead include their reliance on effectively tracking world state and often prohibitively slow run-times ~\cite{garretttamp}. 

In this work, we propose a method to use the online output of TAMP solvers as the target for deep imitation learning. Similar design patterns have effectively learned motor control policies~\cite{GPS}, visuomotor skills~\cite{Finn16}, and classical planning problems~\cite{groshevTamar}. The hope is to train an end-to-end policy that emulates the planner without its computational overhead or need to track the world. To do so, we identify and address three roadblocks: 1) the computational cost of supervision, 2) the complex interplay between abstract actions and controls, and 3) the training-to-test distribution shift.

The first roadblock is that TAMP solvers run substantially slower than the planners used for supervision in the above. To compensate, we train a \emph{motion policy} to imitate the output of a trajectory optimizer, and then initialize trajectory optimization around the output of the policy. As the policy improves, the computational expense to refine each motion plan decreases. To further amplify data generation, our algorithm decomposes across parallelized nodes. The distributed structure allows us to scale our system to utilize all available hardware.

The second roadblock is that mapping from abstract goals to motor controls can require sharp transitions in control space for relatively minor changes in observations. Our system uses the domain-specific TAMP hierarchy in the architecture of the final policy to handle these transitions. We train a \emph{task policy} to output an abstract action to take (e.g., grasp) and associated parameters (e.g., the target object). The motion policy executes conditioned on these outputs. Together the two policies map observations and goals to low-level controls.

The final roadblock is distribution shift. As the time horizons increase, the policies become more likely to deviate from their supervision. We use our policy structure to adopt an active learning (AL) procedure that can be viewed as a hierarchical variant of Dataset Aggregation (DAgger)~\cite{DAgger}. We sample rollouts of the motion policy and augment trajectory optimization with a penalty for deviating from those rollouts. The penalty encourages the optimizer to provide controls similar to those from the policy, akin to DAgger at the motion level. The task planner then samples states where the task policy violates action pre- or post- conditions. The choice of these states focuses demonstrations to where the task policy and expert disagree, akin to DAgger in the abstract space.

The overall contributions of this work are as follows: 1) a method to accelerate task and motion planning via learning motion policies to map parameterized actions to controls and using that policy to amortize trajectory optimization; 2) placing this process inside a parallelized imitation learning framework to train both the motion policies and a goal-conditioned task policy to predict parameterized actions; 3) extending this framework to allow for active learning via the structure of the TAMP problem; and 4) evaluation of the system in a suite of pick-place domains and show that it is capable of learning to accomplish goals over (comparatively) long horizons with both high-dimension sensor data and high-dimension action spaces (e.g. 7-DOF joint control). Our approach uses established machine learning and builds on standard robotics tools. We believe it has the promise to bridge the divide between classical planning and policy learning for robot control.  

==> old_misc.tex <==


%\subsection{Hierarchical Policy Learning}
%Our policies follow a variant of the options framework proposed by \citet{optionlearn}. An option in this context is a tuple $o=<\pi_{lo}, \beta, \mathcal{I}>$, where $\pi_{lo}: \mathcal{S} \to \mathcal{A}$ is a policy, $\beta: \mathcal{S} \to [0,1]$ is a termination condition, and $\mathcal{I} \subset \mathcal{S}$ is the set of states from which $\pi_{lo}$ may be invoked. A high-level policy $\pi_{hi}$ is trained to select the next option $o$. The corresponding $\pi_{lo}$ then executes until termination, at which point $\pi_{hi}$ is re-invoked. The TAMP formalization lends itself naturally to such a framework, with intuitive correspondence from task planning to the selection of $o$ and motion planning to the execution of the respective $\pi^{lo}$. We leverage this abstraction to decouple training of the high-level policy $\pi_{hi}$ and low-level policy $\pi_{lo}$. The termination conditions are implicitly captured in the training for $\pi_{hi}$. To provide additional guidance for $\pi_{lo}$, we augment $\pi_{hi}$ in a manner similar to that of \citet{guidetamp}, using a policy to predict both next $a \in A$ and a onehot-encoding of $a.params$.

%\subsection{Deep Learning for Task and Motion Planning}

%Applying deep learning to long horizon planning has attracted significant interest in recent years ~\cite{vin, symrl, learnsample, pin, upn}. Hierarchical policy structures in particular have extended the horizons existing policy-learning methods can handle~\cite{goalpol, hierdistill, decomphier}. 
%And \citet{actorcriticplan} used an actor-critic method trained form past experience for selecting continuous parameters during the search to improve planning efficiency.

%Various works have proposed deep-learning based methods for improving efficiency in the different components of TAMP. Many of these have focused on the high-level search. \citet{scorespace} used a score-space representation to guide the search via transferring knowledge from previous plans. \citet{feasibletamp} learned a classifier to assess motion feasibility and incorporated it as a heuristic into the search.  To improve efficiency in trajectory optimization, \citet{gripsqp} trained neural networks to predict approximate trajectories that transition from a start frame to the goal, and used these approximate solutions to warm-start trajectory optimization. On the flip side, several works have proposed methods to acquire executable policies that emulate components of TAMP. These approaches do not attempt to improve an existing solver. \citet{mctstamp} combined imitation learning of Monte-Carlo Tree Search (MCTS) in an abstract space with deep q-learning in a control space. They did not address parameterized actions or tasks with multiple sub-goals. \citet{dpdl} trained a high-level model to infer symbolic states, and low-level controllers to convert those symbolic states into controls. They did not train a model for predicting abstract actions, so their system required a symbolic planner be invoked at execution time. \citet{geomlearn} learned a high-level policy to predict sequences of discrete action parameterizations and associated continuous values. For each action, they used model predictive control (MPC) to build transitions around a set of pre-computed trajectories and train a corresponding controller. Their system prioritized joint reasoning over full action sequences and would produce the discrete actions at the start of execution, only updating continuous values between actions.



In this work we propose a method for training goal-conditioned hierarchical policies via imitation of task and motion planning, and demonstrate the ability of the resulting policies to solve complex long-horizon tasks with high-dimensional sensory inputs and control spaces. Our method is able to create a symbiotic relation between learned policies and the TAMP solver, allowing the policies to accelerate the plan refinement process and in turn accelerating the generation of training supervision. The parallelized nature of our algorithms inherently allow them to scale with available hardware, making the system particularly well-suited to industrial environments where many robots operate simultaneously. And we provide empirical validation of both our policy structure and our methods for handling distribution shift of the learned policies - results which can help guide extensions and generalizations of this approach to new planners and environments.


==> tables/sawyerexps.tex <==

\begin{wraptable}{r}{0.35\textwidth}
\vspace{-10pt}
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Method &  1 Object & 2 Object \\
 \hline
 flat-IL & 88\% & 4\%\\
 
no-feedback & 58\% & 14\%\\

task-feedback  & 96\% & 71\% \\

motion-feedback & 97\% & 89\% \\

tamp-feedback & 97\% & 90\% \\
 \hline
\end{tabular}
\caption{Comparison of average goal achievement at the end of training for variants of our system in the RoboSuite benchmark.}
\label{fig:sawyerexp}
\vspace{-10pt}
\end{wraptable}
